Learning Global Transparent Models Consistent with Local Contrastive Explanations

There is a rich and growing literature on producing local contrastive/counterfactual explanations for black-box models (e.g. neural networks). In these methods, for an input, an explanation is in the form of a contrast point differing in very few features from the original input and lying in a different class. Other works try to build globally interpretable models like decision trees and rule lists based on the data using actual labels or based on the black-box models predictions. Although these interpretable global models can be useful, they may not be consistent with local explanations from a specific black-box of choice. In this work, we explore the question: Can we produce a transparent global model that is simultaneously accurate and consistent with the local (contrastive) explanations of the black-box model? We introduce a natural local consistency metric that quantifies if the local explanations and predictions of the black-box model are also consistent with the proxy global transparent model. Based on a key insight we propose a novel method where we create custom boolean features from sparse local contrastive explanations of the black-box model and then train a globally transparent model on just these, and showcase empirically that such models have higher local consistency compared with other known strategies, while still being close in performance to models that are trained with access to the original data.

==> Global Boolean Feature Learning through Contrastive Explanations/macros.tex <==
%\newlength{\dhatheight}
%\newcommand{\doublehat}[1]{%
%    \settoheight{\dhatheight}{\ensuremath{\hat{#1}}}%
%    \addtolength{\dhatheight}{-0.35ex}%
%    \hat{\vphantom{\rule{1pt}{\dhatheight}}%
%    \smash{\hat{#1}}}}

\newlength{\dhatheight}
\newcommand{\hhatDS}[1]{%
    \settoheight{\dhatheight}{\ensuremath{\hat{#1}}}%
    \addtolength{\dhatheight}{-0.35ex}%
    \hat{\vphantom{\rule{1pt}{\dhatheight}}%
    \smash{\hat{#1}}}}
\newcommand{\hhatTS}[1]{%
    \settoheight{\dhatheight}{\ensuremath{\hat{#1}}}%
    \addtolength{\dhatheight}{-0.35ex}%
    \hat{\vphantom{\rule{1pt}{\dhatheight}}%
    \smash{\hat{#1}}}}    
\newcommand{\hhatS}[1]{%
    \settoheight{\dhatheight}{\ensuremath{\scriptstyle{\hat{#1}}}}%
    \addtolength{\dhatheight}{-0.175ex}%
    \hat{\vphantom{\rule{1pt}{\dhatheight}}%
    \smash{\hat{#1}}}}
\newcommand{\hhatSS}[1]{%
    \settoheight{\dhatheight}{\ensuremath{\scriptscriptstyle{\hat{#1}}}}%
    \addtolength{\dhatheight}{-0.07ex}%
    \hat{\vphantom{\rule{1pt}{\dhatheight}}%
    \smash{\hat{#1}}}}
\newcommand{\hhat}[1]{\mathchoice{\hhatDS{#1}}{\hhatTS{#1}}{\hhatS{#1}}{\hhatSS{#1}}}

\newcommand{\region}{\mathcal{U}}
\newcommand{\Px}{\mathcal{P}}
\newcommand{\PXY}{\mathcal{P}_{XY}}
\newcommand{\PXYR}[1]{\mathcal{P}_{#1}}
%\newcommand{\PXYR}{\mathcal{P}_{\region}}
\newcommand{\Risk}{{\rm R}_{\loss}}
\newcommand{\Rademacher}{\hat{\phi}}
\newcommand{\loss}{\ell} % loss function
\newcommand{\maxloss}{\bar{\loss}} % largest possible loss value
\newcommand{\transform}{\psi_{\loss}} % the psi-transform
\newcommand{\tsyba}{\alpha} % Tsybakov exponent for 0-1 loss
\newcommand{\tsybca}{a} % Tsybakov leading constant for 0-1 loss
\newcommand{\tsybb}{\beta} % Tsybakov exponent for surrogate loss
\newcommand{\tsybcb}{b} % Tsybakov leading constant for surrogate loss
\newcommand{\TN}{{\rm MT}} % set of distributions satisfying Tsybakov noise
\newcommand{\BN}{{\rm BN}} % set of distributions satisfying Bounded noise
\newcommand{\RE}{{\rm RE}} % set of distributions satisfying the Realizable case
\newcommand{\AG}{{\rm AG}} % set of distributions satisfying a noise bound in the agnostic case
\newcommand{\BE}{{\rm BE}} % set of distributions satisfying a noise bound in the benign noise case 
\newcommand{\DL}{{\rm BC}} % set of distributions satisfying the diameter localization condition (Bernstein Class Assumption)
\newcommand{\RR}{{\rm RR}} % set of distributions from the work of Raginsky and Rakhlin, 2011
\newcommand{\s}{\mathfrak{s}}
\newcommand{\XTD}{{\rm XTD}} % extended teaching dimension
\newcommand{\TD}{{\rm TD}} % teaching dimension
\newcommand{\XPTD}{{\rm XPTD}} % extended partial teaching dimension
\newcommand{\entc}{q} % leading constant for entropy condition
\newcommand{\entrho}{\rho} % exponent for entropy condition
\newcommand{\g}{g} % a function
\newcommand{\h}{h} % a function (often a classifier)
\newcommand{\f}{f} % another function
\newcommand{\dc}{\theta} % the disagreement coefficient
\newcommand{\zc}{\varphi} % the sup of the ratio of the quantity from 
%\newcommand{\zc}{\sigma} % the sup of the ratio of the quantity from.  (old notation was \varphi, but I noticed Kamalika used \sigma in a talk)
\newcommand{\maxzc}{\hat{\zc}} % the maximum of \zc over the choice of \agtarget
\newcommand{\subcs}{\chi} % subregion compression set size
\newcommand{\ZC}{{\rm SubregionActive}} % subregion-based active learning algorithm
\newcommand{\supdc}{\hhat{\dc}} % the supremum (over distributions and targets) of the disagreement coefficient
\newcommand{\infsplit}{\hhat{\rho}} % infimum splitting index
\newcommand{\basicsplit}{\bar{\rho}} % the splitting index, without the Delta things, just that \C is (\rho,\eps,\tau)-splittable.
%\newcommand{\finitesplit}{\mathring{\rho}} % the limiting splitting index for a finitely discrete distribution
%\newcommand{\uniquesplit}{\sigma} % a variant of splitting where we specify one point responsible for each pair
\newcommand{\dd}{D} % doubling dimension (not sure what a good notation for this might be)
\newcommand{\capacity}{\tau} % the general capacity function
\newcommand{\mixcap}{\chi} % mixed capacity, where the numerator is prob of disagreement while denominator is loss diameter
\newcommand{\exreals}{\bar{\mathbb{R}}}
%\newcommand{\G}{\mathcal{G}}
\newcommand{\J}{{\rm J}} % entropy integral from van der Vaart & Wellner 2011
\newcommand{\D}{{\rm D}} % loss diameter ; might alternatively consider the notation \sigma for this?
\newcommand{\dist}{\Delta} % \Px(x : sign(g(x)) neq sign(h(x)))
\newcommand{\radius}{{\rm radius}} % max distance from target
\newcommand{\Transform}{\Gamma_{\loss}} %%% \Transform(er(h) - er(f*);P) \leq R(h;P) - R(f*;P)
\newcommand{\Epsilon}{\mathscr{E}}
\newcommand{\InvTransform}{\Epsilon_{\loss}}
\newcommand{\Functions}{\F^{*}} % set of all functions
\newcommand{\FunctionsXY}{\G^{*}} % set of functions mapping \X\times\Y \to [-\maxloss,\maxloss].
\newcommand{\Env}{{\rm F}} % envelope function
\newcommand{\bound}{\beta} % the noise bound for bounded noise
\newcommand{\BJM}{\Psi_{\loss}}
\newcommand{\zo}{{\scriptscriptstyle{01}}}
%\newcommand{\targtrunc}[2]{{#1}_{#2}^{\star}}
%\newcommand{\sgntrunc}[2]{{#1}_{#2}^{\pm}}
\newcommand{\spec}[1]{\mathring{#1}} % new special type of bound
\newcommand{\loose}[1]{\breve{#1}} % looser spec bound
\newcommand{\phiinv}[1]{\ddot{#1}} % just invert the phi term for sample size
\newcommand{\restinv}[1]{\dot{#1}} % inverse of the rest of the bound
\newcommand{\ERM}{{\rm ERM}}
\newcommand{\LC}{\Lambda} % label complexity in the pool-based (or stream-based) active learning model
\newcommand{\SC}{\mathcal{M}} % sample complexity of passive learning
\newcommand{\QC}{Q} % query complexity in the repeated query model
%\newcommand{\SC}{{\rm M}}
%\newcommand{\vc}{d}
\newcommand{\vc}{{\rm vc}}
\renewcommand{\dim}{d} % to be introduced as short-hand for VC dimension
\newcommand{\cs}{n} % sample compression size
\newcommand{\covering}{{\cal{N}}}
%\newcommand{\G}{{\cal{G}}}
\newcommand{\conv}{{\rm conv}}
\newcommand{\Fbound}{\bar{B}} % bound on the functions
\newcommand{\metricbound}{\bar{d}_{\loss}} % bound on the pseudo-metric
\newcommand{\metric}{d_{\loss}} % pseudo-metric for the function values
\newcommand{\Lip}{L} % Lipschitz constant
\newcommand{\convc}{C_{\loss}} % constant factor in modulus of convexity lower bound
\newcommand{\convr}{r_{\loss}} % exponent in modulus of convexity lower bound
\newcommand{\modconv}{\bar{\delta}_{\loss}} % modulus of convexity
\newcommand{\Bracket}[1]{[#1]} % bracketing set given by upper and lower envelope functions
\newcommand{\Log}{{\rm Log}}
\newcommand{\polylog}{{\rm polylog}}
\newcommand{\Borel}{{\cal B}}
\newcommand{\BorelX}{{\cal B}_{\X}}

\newcommand{\CAL}{{\rm CAL}}
\newcommand{\ACAL}{RobustCAL}
\newcommand{\Shattering}{Shattering}
\newcommand{\RobustShattering}{RobustShattering}
\newcommand{\ZCPassive}{{\rm Algorithm 1}}
\newcommand{\conf}{\delta}
\newcommand{\eps}{\varepsilon}
\newcommand{\sfun}{\mathfrak{s}}
\newcommand{\X}{\mathcal X} % instance space
\renewcommand{\O}{O} % Big-O notation
\newcommand{\Y}{\mathcal Y} % label space
\newcommand{\alg}{\mathbb{A}} % learning algorithm
\renewcommand{\H}{\mathcal H} % hypothesis space
\renewcommand{\L}{\mathcal L} % labeled set
%\newcommand{\U}{\mathcal U} % unlabeled set
\newcommand{\Z}{\mathcal{Z}}
\newcommand{\target}{f^{\star}} % target function
\newcommand{\agtarget}{h^{\star}} % best classifier in the concept space
\newcommand{\cl}{{\rm cl}} % closure
\newcommand{\er}{{\rm er}} % error rate
\newcommand{\core}{\partial} % disagreement core (or shatter core, when raised to a power)
\newcommand{\konst}{k} % the constant factor we lose in the sample complexity statement
\newcommand{\Ball}{{\rm B}}
\newcommand{\ind}{\mathbbm{1}}
\newcommand{\indpm}{\ind^{\pm}}
\newcommand{\hyp}{h} % hypothesis function
\newcommand{\Q}{\mathcal{Q}}
%\newcommand{\C}{\mathbb{C}} % concept space
\newcommand{\A}{\mathcal{A}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\sign}{{\rm sign}} % sign function
\newcommand{\T}{\mathcal T} % complete answer schemes
\renewcommand{\S}{\mathcal S} % generic collection of sets
\renewcommand{\P}{\mathbb P} % also probability
%\newcommand{\I}{\mathit I} % indicator function
%\newcommand{\R}{\mathit R} % overall risk functional
\newcommand{\nats}{\mathbb{N}} % natural numbers
\newcommand{\reals}{\mathbb{R}} % real numbers
\newcommand{\nts}{\mathbb{Z}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Var}{{\rm Var}}
\newcommand{\Data}{\mathcal{Z}}
\newcommand{\DataX}{\mathbb{X}}
\newcommand{\DataY}{\mathbb{Y}}
%\newcommand{\dense}{\bar}
\newcommand{\dense}{} % this does nothing now
%\renewcommand{\alg}{DHM}
%\newcommand{\citet}{\cite}
%\newcommand{\citep}{\cite}
\newcommand{\diam}{{\rm diam}}
\newcommand{\DIS}{{\rm DIS}}
\newcommand{\DISXY}{\overline{\DIS}}
\newcommand{\DISF}{{\rm DISF}}
\newcommand{\DISFXY}{\overline{\DISF}}
\newcommand{\DISV}{D}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\argmin}{\mathop{\rm argmin}}
%\newcommand{\Tsybakov}{{\rm {Tsybakov}}}
%\newcommand{\vc}{d}
\newcommand{\Dset}{\mathbb{D}}
%\renewcommand{\limsup}{\mathop{\rm limsup}}
%\renewcommand{\liminf}{\mathop{\rm liminf}}
\newcommand{\hdc}{\tilde{\theta}} % higher-order disagreement coefficient
\newcommand{\bdim}{\tilde{d}} % shatter dimension
\newcommand{\dprob}{\tilde{\delta}_{f}}
\newcommand{\supp}{{\rm supp}} % the support of a probability measure
\newcommand{\RQCAL}{Algorithm 1} % the layered repeated queries modification of CAL
\newcommand{\Filter}{Subroutine 1} % the subroutine that repeatedly queries in a cell of the partition
\newcommand{\RealizableAlg}{Algorithm 0} % realizable-case algorithm based on repeated (1/2)-nets querying
\newcommand{\MembHalvingII}{{\sc Memb-Halving-2}} % hegedus memb-halving-2 algorithm
\newcommand{\truV}{V^{\star}} % version space consistent with all the target labels, even those not queried or noisy ones
\newcommand{\Split}{{\rm Split}} % for the splitting index definition
\renewcommand{\a}{a} % constant
\renewcommand{\b}{b} % constant
\renewcommand{\c}{c} % constant

\newcommand{\ignore}[1]{}
\newcommand{\todo}[1]{}
\newcommand{\oldstuff}[1]{}


%\newtheorem{theorem}{Theorem}
%\newtheorem{definition}{Definition}[chapter]
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{definition}[theorem]{Definition}
%\theoremstyle{remark}
%\newtheorem{rem}{Remark}[section]
%\newtheorem{assumption}[theorem]{Assumption}
%\newtheorem{condition}[theorem]{Condition}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{conjecture}[theorem]{Conjecture}

\newsavebox{\savepar}
\newenvironment{bigboxit}{\begin{center}\begin{lrbox}{\savepar}
%\begin{minipage}[h]{5.2in}
\begin{minipage}[h]{3.15in}
%\sffamily
\normalfont
\begin{flushleft}}
{\end{flushleft}\end{minipage}\end{lrbox}\fbox{\usebox{\savepar}}
\end{center}}

\newenvironment{bigbigboxit}{\begin{center}\begin{lrbox}{\savepar}
%\begin{minipage}[h]{5.2in}
\begin{minipage}[h]{5.8in}
%\sffamily
\normalfont
\begin{flushleft}}
{\end{flushleft}\end{minipage}\end{lrbox}\fbox{\usebox{\savepar}}
\end{center}}


\makeatletter
\newcommand{\vast}{\bBigg@{3}}
\newcommand{\Vast}{\bBigg@{4}}
\makeatother


==> macros.tex <==
%\newlength{\dhatheight}
%\newcommand{\doublehat}[1]{%
%    \settoheight{\dhatheight}{\ensuremath{\hat{#1}}}%
%    \addtolength{\dhatheight}{-0.35ex}%
%    \hat{\vphantom{\rule{1pt}{\dhatheight}}%
%    \smash{\hat{#1}}}}

\newlength{\dhatheight}
\newcommand{\hhatDS}[1]{%
    \settoheight{\dhatheight}{\ensuremath{\hat{#1}}}%
    \addtolength{\dhatheight}{-0.35ex}%
    \hat{\vphantom{\rule{1pt}{\dhatheight}}%
    \smash{\hat{#1}}}}
\newcommand{\hhatTS}[1]{%
    \settoheight{\dhatheight}{\ensuremath{\hat{#1}}}%
    \addtolength{\dhatheight}{-0.35ex}%
    \hat{\vphantom{\rule{1pt}{\dhatheight}}%
    \smash{\hat{#1}}}}    
\newcommand{\hhatS}[1]{%
    \settoheight{\dhatheight}{\ensuremath{\scriptstyle{\hat{#1}}}}%
    \addtolength{\dhatheight}{-0.175ex}%
    \hat{\vphantom{\rule{1pt}{\dhatheight}}%
    \smash{\hat{#1}}}}
\newcommand{\hhatSS}[1]{%
    \settoheight{\dhatheight}{\ensuremath{\scriptscriptstyle{\hat{#1}}}}%
    \addtolength{\dhatheight}{-0.07ex}%
    \hat{\vphantom{\rule{1pt}{\dhatheight}}%
    \smash{\hat{#1}}}}
\newcommand{\hhat}[1]{\mathchoice{\hhatDS{#1}}{\hhatTS{#1}}{\hhatS{#1}}{\hhatSS{#1}}}

\newcommand{\region}{\mathcal{U}}
\newcommand{\Px}{\mathcal{P}}
\newcommand{\PXY}{\mathcal{P}_{XY}}
\newcommand{\PXYR}[1]{\mathcal{P}_{#1}}
%\newcommand{\PXYR}{\mathcal{P}_{\region}}
\newcommand{\Risk}{{\rm R}_{\loss}}
\newcommand{\Rademacher}{\hat{\phi}}
\newcommand{\loss}{\ell} % loss function
\newcommand{\maxloss}{\bar{\loss}} % largest possible loss value
\newcommand{\transform}{\psi_{\loss}} % the psi-transform
\newcommand{\tsyba}{\alpha} % Tsybakov exponent for 0-1 loss
\newcommand{\tsybca}{a} % Tsybakov leading constant for 0-1 loss
\newcommand{\tsybb}{\beta} % Tsybakov exponent for surrogate loss
\newcommand{\tsybcb}{b} % Tsybakov leading constant for surrogate loss
\newcommand{\TN}{{\rm MT}} % set of distributions satisfying Tsybakov noise
\newcommand{\BN}{{\rm BN}} % set of distributions satisfying Bounded noise
\newcommand{\RE}{{\rm RE}} % set of distributions satisfying the Realizable case
\newcommand{\AG}{{\rm AG}} % set of distributions satisfying a noise bound in the agnostic case
\newcommand{\BE}{{\rm BE}} % set of distributions satisfying a noise bound in the benign noise case 
\newcommand{\DL}{{\rm BC}} % set of distributions satisfying the diameter localization condition (Bernstein Class Assumption)
\newcommand{\RR}{{\rm RR}} % set of distributions from the work of Raginsky and Rakhlin, 2011
\newcommand{\s}{\mathfrak{s}}
\newcommand{\XTD}{{\rm XTD}} % extended teaching dimension
\newcommand{\TD}{{\rm TD}} % teaching dimension
\newcommand{\XPTD}{{\rm XPTD}} % extended partial teaching dimension
\newcommand{\entc}{q} % leading constant for entropy condition
\newcommand{\entrho}{\rho} % exponent for entropy condition
\newcommand{\g}{g} % a function
\newcommand{\h}{h} % a function (often a classifier)
\newcommand{\f}{f} % another function
\newcommand{\dc}{\theta} % the disagreement coefficient
\newcommand{\zc}{\varphi} % the sup of the ratio of the quantity from 
%\newcommand{\zc}{\sigma} % the sup of the ratio of the quantity from.  (old notation was \varphi, but I noticed Kamalika used \sigma in a talk)
\newcommand{\maxzc}{\hat{\zc}} % the maximum of \zc over the choice of \agtarget
\newcommand{\subcs}{\chi} % subregion compression set size
\newcommand{\ZC}{{\rm SubregionActive}} % subregion-based active learning algorithm
\newcommand{\supdc}{\hhat{\dc}} % the supremum (over distributions and targets) of the disagreement coefficient
\newcommand{\infsplit}{\hhat{\rho}} % infimum splitting index
\newcommand{\basicsplit}{\bar{\rho}} % the splitting index, without the Delta things, just that \C is (\rho,\eps,\tau)-splittable.
%\newcommand{\finitesplit}{\mathring{\rho}} % the limiting splitting index for a finitely discrete distribution
%\newcommand{\uniquesplit}{\sigma} % a variant of splitting where we specify one point responsible for each pair
\newcommand{\dd}{D} % doubling dimension (not sure what a good notation for this might be)
\newcommand{\capacity}{\tau} % the general capacity function
\newcommand{\mixcap}{\chi} % mixed capacity, where the numerator is prob of disagreement while denominator is loss diameter
\newcommand{\exreals}{\bar{\mathbb{R}}}
%\newcommand{\G}{\mathcal{G}}
\newcommand{\J}{{\rm J}} % entropy integral from van der Vaart & Wellner 2011
\newcommand{\D}{{\rm D}} % loss diameter ; might alternatively consider the notation \sigma for this?
\newcommand{\dist}{\Delta} % \Px(x : sign(g(x)) neq sign(h(x)))
\newcommand{\radius}{{\rm radius}} % max distance from target
\newcommand{\Transform}{\Gamma_{\loss}} %%% \Transform(er(h) - er(f*);P) \leq R(h;P) - R(f*;P)
\newcommand{\Epsilon}{\mathscr{E}}
\newcommand{\InvTransform}{\Epsilon_{\loss}}
\newcommand{\Functions}{\F^{*}} % set of all functions
\newcommand{\FunctionsXY}{\G^{*}} % set of functions mapping \X\times\Y \to [-\maxloss,\maxloss].
\newcommand{\Env}{{\rm F}} % envelope function
\newcommand{\bound}{\beta} % the noise bound for bounded noise
\newcommand{\BJM}{\Psi_{\loss}}
\newcommand{\zo}{{\scriptscriptstyle{01}}}
%\newcommand{\targtrunc}[2]{{#1}_{#2}^{\star}}
%\newcommand{\sgntrunc}[2]{{#1}_{#2}^{\pm}}
\newcommand{\spec}[1]{\mathring{#1}} % new special type of bound
\newcommand{\loose}[1]{\breve{#1}} % looser spec bound
\newcommand{\phiinv}[1]{\ddot{#1}} % just invert the phi term for sample size
\newcommand{\restinv}[1]{\dot{#1}} % inverse of the rest of the bound
\newcommand{\ERM}{{\rm ERM}}
\newcommand{\LC}{\Lambda} % label complexity in the pool-based (or stream-based) active learning model
\newcommand{\SC}{\mathcal{M}} % sample complexity of passive learning
\newcommand{\QC}{Q} % query complexity in the repeated query model
%\newcommand{\SC}{{\rm M}}
%\newcommand{\vc}{d}
\newcommand{\vc}{{\rm vc}}
\renewcommand{\dim}{d} % to be introduced as short-hand for VC dimension
\newcommand{\cs}{n} % sample compression size
\newcommand{\covering}{{\cal{N}}}
%\newcommand{\G}{{\cal{G}}}
\newcommand{\conv}{{\rm conv}}
\newcommand{\Fbound}{\bar{B}} % bound on the functions
\newcommand{\metricbound}{\bar{d}_{\loss}} % bound on the pseudo-metric
\newcommand{\metric}{d_{\loss}} % pseudo-metric for the function values
\newcommand{\Lip}{L} % Lipschitz constant
\newcommand{\convc}{C_{\loss}} % constant factor in modulus of convexity lower bound
\newcommand{\convr}{r_{\loss}} % exponent in modulus of convexity lower bound
\newcommand{\modconv}{\bar{\delta}_{\loss}} % modulus of convexity
\newcommand{\Bracket}[1]{[#1]} % bracketing set given by upper and lower envelope functions
\newcommand{\Log}{{\rm Log}}
\newcommand{\polylog}{{\rm polylog}}
\newcommand{\Borel}{{\cal B}}
\newcommand{\BorelX}{{\cal B}_{\X}}

\newcommand{\CAL}{{\rm CAL}}
\newcommand{\ACAL}{RobustCAL}
\newcommand{\Shattering}{Shattering}
\newcommand{\RobustShattering}{RobustShattering}
\newcommand{\ZCPassive}{{\rm Algorithm 1}}
\newcommand{\conf}{\delta}
\newcommand{\eps}{\varepsilon}
\newcommand{\sfun}{\mathfrak{s}}
\newcommand{\X}{\mathcal X} % instance space
\renewcommand{\O}{O} % Big-O notation
\newcommand{\Y}{\mathcal Y} % label space
\newcommand{\alg}{\mathbb{A}} % learning algorithm
\renewcommand{\H}{\mathcal H} % hypothesis space
\renewcommand{\L}{\mathcal L} % labeled set
%\newcommand{\U}{\mathcal U} % unlabeled set
\newcommand{\Z}{\mathcal{Z}}
\newcommand{\target}{f^{\star}} % target function
\newcommand{\agtarget}{h^{\star}} % best classifier in the concept space
\newcommand{\cl}{{\rm cl}} % closure
\newcommand{\er}{{\rm er}} % error rate
\newcommand{\core}{\partial} % disagreement core (or shatter core, when raised to a power)
\newcommand{\konst}{k} % the constant factor we lose in the sample complexity statement
\newcommand{\Ball}{{\rm B}}
\newcommand{\ind}{\mathbbm{1}}
\newcommand{\indpm}{\ind^{\pm}}
\newcommand{\hyp}{h} % hypothesis function
\newcommand{\Q}{\mathcal{Q}}
%\newcommand{\C}{\mathbb{C}} % concept space
\newcommand{\A}{\mathcal{A}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\sign}{{\rm sign}} % sign function
\newcommand{\T}{\mathcal T} % complete answer schemes
\renewcommand{\S}{\mathcal S} % generic collection of sets
\renewcommand{\P}{\mathbb P} % also probability
%\newcommand{\I}{\mathit I} % indicator function
%\newcommand{\R}{\mathit R} % overall risk functional
\newcommand{\nats}{\mathbb{N}} % natural numbers
\newcommand{\reals}{\mathbb{R}} % real numbers
\newcommand{\nts}{\mathbb{Z}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Var}{{\rm Var}}
\newcommand{\Data}{\mathcal{Z}}
\newcommand{\DataX}{\mathbb{X}}
\newcommand{\DataY}{\mathbb{Y}}
%\newcommand{\dense}{\bar}
\newcommand{\dense}{} % this does nothing now
%\renewcommand{\alg}{DHM}
%\newcommand{\citet}{\cite}
%\newcommand{\citep}{\cite}
\newcommand{\diam}{{\rm diam}}
\newcommand{\DIS}{{\rm DIS}}
\newcommand{\DISXY}{\overline{\DIS}}
\newcommand{\DISF}{{\rm DISF}}
\newcommand{\DISFXY}{\overline{\DISF}}
\newcommand{\DISV}{D}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\argmin}{\mathop{\rm argmin}}
%\newcommand{\Tsybakov}{{\rm {Tsybakov}}}
%\newcommand{\vc}{d}
\newcommand{\Dset}{\mathbb{D}}
%\renewcommand{\limsup}{\mathop{\rm limsup}}
%\renewcommand{\liminf}{\mathop{\rm liminf}}
\newcommand{\hdc}{\tilde{\theta}} % higher-order disagreement coefficient
\newcommand{\bdim}{\tilde{d}} % shatter dimension
\newcommand{\dprob}{\tilde{\delta}_{f}}
\newcommand{\supp}{{\rm supp}} % the support of a probability measure
\newcommand{\RQCAL}{Algorithm 1} % the layered repeated queries modification of CAL
\newcommand{\Filter}{Subroutine 1} % the subroutine that repeatedly queries in a cell of the partition
\newcommand{\RealizableAlg}{Algorithm 0} % realizable-case algorithm based on repeated (1/2)-nets querying
\newcommand{\MembHalvingII}{{\sc Memb-Halving-2}} % hegedus memb-halving-2 algorithm
\newcommand{\truV}{V^{\star}} % version space consistent with all the target labels, even those not queried or noisy ones
\newcommand{\Split}{{\rm Split}} % for the splitting index definition
\renewcommand{\a}{a} % constant
\renewcommand{\b}{b} % constant
\renewcommand{\c}{c} % constant

\newcommand{\ignore}[1]{}
\newcommand{\todo}[1]{}
\newcommand{\oldstuff}[1]{}


%\newtheorem{theorem}{Theorem}
%\newtheorem{definition}{Definition}[chapter]
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{definition}[theorem]{Definition}
%\theoremstyle{remark}
%\newtheorem{rem}{Remark}[section]
%\newtheorem{assumption}[theorem]{Assumption}
%\newtheorem{condition}[theorem]{Condition}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{conjecture}[theorem]{Conjecture}

\newsavebox{\savepar}
\newenvironment{bigboxit}{\begin{center}\begin{lrbox}{\savepar}
%\begin{minipage}[h]{5.2in}
\begin{minipage}[h]{3.15in}
%\sffamily
\normalfont
\begin{flushleft}}
{\end{flushleft}\end{minipage}\end{lrbox}\fbox{\usebox{\savepar}}
\end{center}}

\newenvironment{bigbigboxit}{\begin{center}\begin{lrbox}{\savepar}
%\begin{minipage}[h]{5.2in}
\begin{minipage}[h]{5.8in}
%\sffamily
\normalfont
\begin{flushleft}}
{\end{flushleft}\end{minipage}\end{lrbox}\fbox{\usebox{\savepar}}
\end{center}}


\makeatletter
\newcommand{\vast}{\bBigg@{3}}
\newcommand{\Vast}{\bBigg@{4}}
\makeatother

